Emergence of curved momentum-spacetime and its effect on the cyclotron motion in the antiferromagnetic quantum critical metal

We show that anisotropic quantum corrections can dynamically give rise to curved momentum-spacetimes for quasiparticles in metals. In the (2+1)-dimensional antiferromagnetic quantum critical metal, a curved momentum-spacetime arises as the critical spin fluctuations generate red shift that dilates frequency of electron unevenly on the Fermi surface. As the disparity of the momentum-dependent red shift is controlled by the shape of the Fermi surface, the momentum-spacetime geometry that emerges at low energies depends on the bare nesting angle of the Fermi surface. With increasing nesting angle, the region in which electron motion is slowed down by critical spin fluctuations shrinks. On the other hand, the increasing nesting angle makes the red shift stronger near the hot spots due to the weakened screening of the interaction. These competing effects result in a non-monotonic dependence of the cyclotron frequency of electron on the nesting angle of the Fermi surface. The red shift that becomes more singular at the hot spots with increasing nesting angle creates a possibility of realizing a momentum-space black hole horizon beyond a critical nesting angle : the electron motion becomes `perpetually' slowed down as it approaches a hot spot in the same way that the motion of a free falling object freezes near the event horizon of a black hole with respect to an asymptotic observer. However, the analogous horizon in momentum space does not lead to a vanishing cyclotron frequency because the metric singularity at the hot spots is cut off by thermal effects present above the non-zero superconducting transition temperature.

==> notes.tex <==
\section{Notes}
%
%We want to describe the motion of a narrow wave packet obtained by superposing the Bloch states of a band (no inter-band transitions.)
%
%Emergent quantities in the wave packet approach: orbital magnetic moment of the wave packet and  dipole moment of the wave packet.

%The general, unperturbed wave packet is
%\begin{equation}
%\ket{W_0} = \int \dd^d q w(\vec{q},t)\ket{\psi_n(\vec{q})},
%\end{equation}
%where $\psi_n$ are the Bloch functions from the $n$-th band and $w(\vec{q},t)$ is the envelope function. The properties of $w$ are
%\begin{itemize}
%\item $w(\vec{q},t)$ must have a sharp distribution in the BZ such that it makes sense to speak about the wave vector $\vec{q}_c = \int \dd^d q \vec{q}\abs{w(\vec{q},t)}^2$.
%
%To first order, $\abs{w(\vec{q},t)}^2 \approx \delta(\vec{q} - \vec{q}_c)$ ($\int \dd^d qf(\vec{q})\abs{w(\vec{q},t)}^2 \approx f(\vec{q}_c)$.)
%
%\item The packet has to be narrowly localized near its center of mass $\vec{r}_c = \mel{W_0}{\vec{r}}{W_0}$.
%
%In general,
%\begin{equation}
%\vec{r}_c = -\vec{\nabla}_{\vec{q}_c}\arg{w(\vec{q}_c,t)} +\mathcal{A}^{n}_{\vec{q}}(\vec{q}_c),
%\end{equation}
%where $\mathcal{A}^{n}_{\vec{q}} = i \mel{u_n(\vec{q})}{\vec{\nabla}_{\vec{q}}}{u_n(\vec{q})}$ is the Berry connection and $u_n(\vec{q})$ are the Bloch waves. The pair $\vec{r}_c, \vec{q}_c$ are the wave packet center.
%\end{itemize}

%Omitting the subscript $c$ from now on, the general Lagrangian for phase space evolution of the center of the wave packet $(\vec{r}, \vec{k})$ is 
%\begin{equation}
%L = \vec{k}\cdot \dot{\vec{r}} - \varepsilon_M(\vec{k}) + e \phi(\vec{r}) - e \dot{\vec{r}}\cdot\vec{A}(\vec{r},t) + \dot{\vec{k}}\cdot \mathcal{A}_n(\vec{k}),
%\end{equation}
%where $\varepsilon_M(\vec{k}) = \varepsilon_0(\vec{k}) - \vec{B}\cdot\vec{m}(\vec{k})$, $\vec{m}(\vec{k})$ is the orbital moment, and $\phi(\vec{r})$ and $\vec{A}(\vec{r},t)$ are the electromagnetic potentials. We want to describe the dynamics of the simplest wave packet first. We only assume a perturbation by a external magnetic field and no electric field (no free currents) and uniform charge distribution (no bound currents) ($\vec{m}(\vec{k}) = \vec{0}$), and finally, we ignore the Berry curvature for the moment.
%
%The equations of motion for this case are:
%\begin{subequations}
%\begin{align}
%\dot{\vec{r}} = & \vec{\nabla}_{\vec{k}}\varepsilon_0(\vec{k}) = \vec{v}_0(\vec{k}),
%\label{eq:rdot}
%\\ \dot{\vec{k}} = & -e \dot{\vec{r}}\times{\vec{B}},
%\label{eq:kdot}
%\end{align}
%where $\vec{v}_0(\vec{k})$ is the group velocity of the wave packet.
%\end{subequations}


\subsection{Zero Energy Limit}

Let us analyze the movement of the wavepacket as it traverses the Fermi surface relative to hot spot 1 in the low energy limit (see Figure \ref{fig:setup}). We choose $\vec{B} = B_0 \hat{z}$, i.e. in the direction perpendicular to the Fermi sea plane. The frame of reference is attached to the hot spot and all momentum is measured relative to it. In the low energy limit, $\varepsilon_0(\vec{k}) = \vec{v}_F(\vec{k})\cdot{\vec{k}}$, where $\vec{v}_F(\vec{k}) = \mathcal{V}_{F,k}\left(v_{0}(0)\hat{x}+\hat{y}\right)$ is the (vector) Fermi velocity. Here, $k = k_x$ to simplify notation. $ \mathcal{V}_{F,k}$ is the Fermi velocity along $\hat{y}$

we will simply call it Fermi velocity. 
\begin{equation}
k_c = \frac{\Lambda}{4 v_0(0)}
\end{equation}
is the momentum at the end of the integration region, called ``cold momentum'' and $k_h =0$ is the hot spot momentum, or ``hot momentum''. The exponent $\alpha_1(0)$ is a critical exponent,

where $\ell$ is the length scale.
$\mathcal{V}_{F,k}v_0(0)$ is the Fermi velocity in $\hat{\bf{x}}$, where

is the nesting at momentum $k$ and length scale $\ell$, which describes the curvature of the Fermi surface at $k$ at the energy scale $\Lambda e^{-\ell}$. In the zero energy limit we have $\ell, \ell_0 \gg 1$, which we call the ``low energy limit'' and $\ell/\ell_0 \ll 1$. Therefore, we can ignore the flow of $v$, i.e. $v_k(\ell) \approx v_0(0)$.

The equations of motion are

Separating Eq. \eqref{eq:kdotlowe} in components:

The equation for $k_y$ has the formal solution
\begin{equation}
k_y(t) = k_y(0) + \frac{e B_0 v_0(0)}{k_c^{\alpha_1(0)}}\int_0^t \abs{k(t')}^{\alpha_1(0)} \mathrm{d}t'.
\label{eq:kyeq}
\end{equation}

Since $k_c = \frac{\Lambda}{4 v_0(0)}$ depends on $\ell_0$, we can solve the equation for $k$ under two types of initial conditions: (1) For $k(0) = k_c$ and (2) $k(0) = k_0 > 0$ fixed for all $\ell_0$. For case (1), the solution is
\begin{equation}
\frac{k(t)}{k_c} = \left\lbrace\begin{matrix}
\left(1 - \frac{t}{t_{hs}}\right)^{\frac{1}{1-\alpha_1(0)}}, & 0< t \leq t_{hs},
\\ -\left(\frac{t}{t_{hs}} - 1\right)^{\frac{1}{1-\alpha_1(0)}}, & t_{hs} < t \leq t_f ,
\end{matrix}\right. ,
\label{eq:solkc}
\end{equation}
where
\begin{equation}
t_{hs} = \frac{k_c}{(1-\alpha_1(0))e B_0}
\label{eq:thskc}
\end{equation}
is the time taken to reach the hot spot and $t_f = 2t_{hs}$ is the time to reach the other edge, i.e. $k(t_f) = -k_c$. In case (2), the solution is
\begin{equation}
\frac{k(t)}{k_0} = \left\lbrace\begin{matrix}
\left(1 - \frac{t}{t^{(0)}_{hs}}\right)^{\frac{1}{1-\alpha_1(0)}}, & 0< t \leq t^{(0)}_{hs},
\\ -\left(\frac{t}{t^{(0)}_{hs}} - 1\right)^{\frac{1}{1-\alpha_1(0)}}, & t^{(0)}_{hs} < t \leq t^{(0)}_f ,
\end{matrix}\right. ,
\label{eq:solk0}
\end{equation}
where
\begin{equation}
t^{(0)}_{hs} = \frac{k_0}{(1-\alpha_1(0))e B_0}\left(\frac{k_c}{k_0}\right)^{\alpha_1(0)}
\label{eq:thsk0}
\end{equation}
is the time to reach the hot spot and 
\begin{equation}
t^{(0)}_f = t^{(0)}_{hs} + t_{hs}
\label{eq:tfk0}
\end{equation}
is the time to reach the other edge, $k(t^{(0)}_f) = -k_c$. The time to reach $-k_0$ (instead of $-k_c$) is $2 t^{(0)}_{hs}$.

Using Eq. \eqref{eq:ellzero}, we can see that the low energy limit, $\ell_0 \to \infty$ is equivalent to the limit $v_0(0) \to 0$. However, a word of caution is that the strict equality $v_0(0) = 0$ is never taken. in the small $v_0(0)$ limit, the time $t_{hs}$ is
\begin{equation}
t_{hs} \approx \frac{\Lambda}{4 e B_0}\left[\frac{1}{v_0(0)} + \frac{\sqrt{2}(N_c^2 - 1)}{\pi \sqrt{N_c N_f}}\frac{\sqrt{\frac{\log(1/v_0(0))}{v_0(0)}}}{\log\left(\frac{\pi^2 N_c N_f}{2(N_c^2 - 1)}\frac{1}{v_0(0)\log(1/v_0(0))}\right)} \right],
\end{equation}
where the second term is subleading in growth. As $v_0(0)$ decreases, the time the wave packet takes to reach the hot spot increases as $1/v_0(0)$. $2 t_{hs}$ also represents 1/8 of the period it takes the wave packet to traverse the whole Fermi surface:
\begin{equation}
\mathrm{T} = 16 t_{hs} \approx \frac{4\Lambda}{e B_0 v_0(0)}. 
\end{equation}
For the initial condition $k(0)=k_0$, the small $v_0(0)$ limit is
\begin{equation}
t^{(0)}_{hs} \approx \frac{k_0}{e B_0}\left[1 + \frac{\sqrt{2}(N_c^2 - 1)}{\pi\sqrt{N_c N_f}}\frac{\sqrt{v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\left(1+\log\left(\frac{\Lambda\log\left(\frac{\pi^2 N_c N_f}{2(N_c^2 - 1)}\frac{1}{v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\right)}{4k_0 v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\right)\right)}{\log\left(\frac{\pi^2 N_c N_f}{2(N_c^2 - 1)}\frac{1}{v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\right)} \right].
\label{eq:ths0exp}
\end{equation}
\begin{figure}[t]
\centering
\includegraphics[width=0.75\linewidth]{zeroesLWk.pdf}
\caption{Numerical plot of time $t^{(0)}_{hs}$ the wave packet takes to reach the hot spot in the region away from the Hot spot. $e = B_0 = 1$ and $\Lambda = 1$. The fixed initial momentum is $k_{0} = 6\Lambda$ and ``hot spot'' momentum is of the order $k^*_{hs} \sim \Lambda 10^{-6}$ for the different values of $\ell_0$ and $k^*_{0}$. Here the wave packet takes less time to reach the hot spot as we move towards the small $v_0(0)$. The saturation value is $t^{(0)}_{hs} = 6$.}
\label{fig:timezeroaway}
\end{figure}
Therefore, in the low energy limit, the time necessary to reach the hot spot from $k_0$ saturates to (See Fig.\ref{fig:timezeroaway})
\begin{equation}
t^{(0)}_{hs} \underset{v_0(0) \to 0}{\approx} \frac{k_0}{e B_0}.
\end{equation}
If we consider $k_0$ and $-k_0$ as the initial and final points of the movement of the wave-packet, then it's period around the
\begin{equation}
\mathrm{T}^{(0)} = 16 t^{(0)}_{hs} \approx \frac{16 k_0}{e B_0}.
\end{equation}
For any of the initial conditions above, Eq. \eqref{eq:kyeq} satisfies
\begin{equation}
k_y(t) = -v_0(0)k(t),
\end{equation}
as long as the initial condition is $k_y(0) = -v_0(0)k(0)$.

\subsection{Approaching the hot spot in the low energy limit}

Let us analyze the solution in Eqs. \eqref{eq:solk0} and \eqref{eq:thsk0} by extending the region in which $\ell$ and $\ell_0$ are comparable\footnote{We can argue that the full zero energy limit is the zeroth order approximation and this extension is equivalent to taking next order corrections in the expansion.}. We do this by defining the momentum $k^*_{hs}$ as the momentum in which the $\ell/\ell_0 \ll 1$ limit breaks down. Here,
\begin{equation}
k^*_{hs} = \frac{\Lambda e^{-\ell_0}}{4 v_0(0)}.
\end{equation}
Below $k^*_{hs}$, we are still taking the low energy limit, but we cannot ignore momentum dependent features of the flow when arbitrarily close to the hot spot\footnote{We are still taking $k_{hs}=0$.}. In other words, we need to consider the full flow of $v_k(\ell)$ and $\mathcal{V}_{F,k}$, i.e.
\begin{equation}
v_k(\ell) = v_0(\ell^{(2L)}_k), \quad \mathcal{V}_{F,k} = \mathcal{E}_1(\ell^{(2L)}_k;0)^{-1} = \exp\left\lbrace\sqrt{N_c^2-1}\left[-\Ei\left(\log\sqrt{\ell^{(2L)}_k + \ell_0}\right)+\Ei\left(\log\sqrt{\ell_0}\right)\right]\right\rbrace,
\end{equation}
where $\ell^{(2L)}_k = \log\left(\frac{\Lambda}{4 v_0(0)\abs{k}}\right)$ is the crossover length scale to the hot region. We will constraint to the movement between $k_0$ and the hot spot.

\subsubsection{$\alpha_1 \ll 1 $ and $\alpha_1 \approx 1$ limits away from the Hot Spot}

 As we reduce $\ell_0$, we decrease the value of $k_c$ and increase $\alpha_1(0)$. Therefore, since $k_0$ is fixed, we have to consider the values of $\ell_0$ for which $k_c > k_0$ and the values for which $k_0 > k_c$. In the case $k_c>k_0$, let us consider a wave packet that travels from $k_0$ to $\varepsilon$, with $k_{h}=0 < k^*_{hs} < \varepsilon < k(t) \ll k_0 (< k_c)$. Here, we just have to solve Eqs. \eqref{eq:dotkaeq}. The time $T_1(\varepsilon,k_0;\ell_0)$ the wave packet takes to arrive to $\varepsilon$ from $k_0$ is
where $t^{(0)}_{hs}$ given by Eq. \eqref{eq:thsk0}. In this region we can still take the $\ell/\ell_0 \ll 1$ limit and we obtain a modified expression of Eq. \eqref{eq:ths0exp} for $T_1(\varepsilon,k_0;\ell_0)$,
\begin{equation}
\begin{aligned}
T_1(\varepsilon,k_0;\ell_0) \approx & \frac{k_0-\varepsilon}{e B_0} + \frac{\sqrt{2}(N_c^2 - 1)}{\pi\sqrt{N_c N_f}}\frac{\sqrt{v_0(0)\log\left(\frac{1}{v_0(0)}\right)}}{\log\left(\frac{\pi^2 N_c N_f}{2(N_c^2 - 1)}\frac{1}{v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\right)}\left[ \frac{k_0-\varepsilon}{e B_0} +\frac{k_0}{e B_0}\log\left(\frac{\Lambda\log\left(\frac{\pi^2 N_c N_f}{2(N_c^2 - 1)}\frac{1}{v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\right)}{4k_0 v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\right)\right. 
\\ & \left. - \frac{\varepsilon}{e B_0}\log\left(\frac{\Lambda\log\left(\frac{\pi^2 N_c N_f}{2(N_c^2 - 1)}\frac{1}{v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\right)}{4\varepsilon v_0(0)\log\left(\frac{1}{v_0(0)}\right)}\right) \right].
\end{aligned}
\label{eq:tepsilonexp}
\end{equation}
In this limit, logarithmic corrections vanish in the small $v_0(0)$/large $\ell_0$ limit, such that it saturates to the positive value
\begin{equation}
T_1(\varepsilon,k_0;\ell_0) \approx \frac{k_0-\varepsilon}{e B_0},
\end{equation}
as expected. Secondly, notice that Eq. \eqref{eq:tepsilon} (and Eq. \eqref{eq:thsk0}) diverge when the critical exponent $\alpha_1(0)$ reaches the critical value $\alpha_1(0) = 1$. 
\begin{figure}[t]
\centering
\includegraphics[width=0.5\linewidth]{uniquesolelectron.pdf}
\caption{Graphical solution of Eq. \eqref{eq:alpha1one} for the case of electrons $N_f = 1, N_c = 2$ (although $N_f = 1$ is not required.) The two curves intersect at $\ell_0 \approx 2.810$.}
\label{fig:uniquesolelectrons}
\end{figure}
For electrons, $N_f = 1, N_c = 2$, there is the unique solution $\ell^{\text{crit}}_0 \approx 2.810$(See Fig. \ref{fig:uniquesolelectrons}), this gives $v_0(0) \approx 1.133$, which is out of the scope of the small nesting angle limit. However, to reach the solution in Eq. \eqref{eq:tepsilon}, we do not require conditions on $k_c$ and $\alpha_1(0)$ other than $\alpha_1(0)\neq 1$. Therefore, let us set $k_c$ to be a fixed, large value of momentum $k_c = k^*_c$ and expand Eq. \eqref{eq:tepsilon} near $\alpha_1(0) = 1$. The result, denoted by $T_1^\star$ to refer to the critical value of $\alpha_1$, is
\begin{equation}
T_1^\star(\varepsilon,k_0;\ell_0 \to\ell^{\text{crit}}_0) = \frac{k^*_c}{e B_0}\log\left(\frac{k_0}{\varepsilon}\right) +\mathcal{O}(1-\alpha_1(0)).
\label{eq:tepsiloncritexp}
\end{equation}
This equation introduces a $\varepsilon$-dependent logarithmic correction to the time it takes the wave packet to arrive to the hot spot region delimited by $k^*_{hs}$. Since $k_0 >\varepsilon$, $T_1^\star(\varepsilon,k_0;\ell^{\text{crit}}_0)$ increases as $\varepsilon$ decreases down to $k^*_{hs}$.

Finally, in the case $k_0>k_c$, we have to solve the equation for two regimes: (1) $k^*_{hs} < \varepsilon < k(t) < k_c (< k_0)$, where the Fermi velocity acquires it ``cold'' value $\mathcal{V}_{F,k} = 1$:
\begin{equation}
\dot{\vec{k}}(t) = -e B_0\left(\hat{x}- v_0(0)\hat{y}\right) \Rightarrow \dot{k}(t) = -e B_0.
\label{eq:coldkeq}
\end{equation}
Then the time to reach $k_c$ from $k_0$ is
\begin{equation}
t(k_c) = \frac{k_0 - k_c}{e B_0}.
\end{equation}
The time to reach $\varepsilon$ from $k_c$ is obtained by solving the Eq. \eqref{eq:dotkaeq} with the initial condition $k(0)=k_c$. The result is
\begin{equation}
\overline{t}(\varepsilon) = t_{hs}\left[1 - \left(\frac{\varepsilon}{k_c}\right)^{1-\alpha_1(0)}\right],
% \label{eq:tepsiloncold}
\end{equation}
where $t_{hs}$ is given in Eq. \eqref{eq:thskc}. The Full time $T_2(\varepsilon,k_0;\ell_0)$ is given by $t(k_c) +\overline{t}(\varepsilon)$. Explicitly,
\begin{equation}
T_2(\varepsilon,k_0;\ell_0) = \frac{k_0}{e B_0} + t_{hs}\left[\alpha_1(0) - \left(\frac{\varepsilon}{k_c}\right)^{1-\alpha_1(0)}\right].
\label{eq:fulltepsiloncold}
\end{equation}

In general, the time it takes the wave packet to reach the hot spot is 
\begin{equation}
T_{12}(\varepsilon,k_0;\ell_0) = \Theta\left(k_c-k_0\right)T_1(\varepsilon,k_0;\ell_0) + \Theta\left(k_0 - k_c\right)T_2(\varepsilon,k_0;\ell_0),
\label{eq:generaltepsilonaway}
\end{equation}
where $\Theta$ is the Heaviside step function and $T_1(\varepsilon,k_0;\ell_0)$ and $T_2(\varepsilon,k_0;\ell_0)$ are given by Eqs. \eqref{eq:tepsilon} and \eqref{eq:fulltepsiloncold}, respectively. The plot in Fig. \ref{fig:fulltimezeroaway} shows the full behaviour of the time to reach the hot spot as a function of the bare scale $\ell_0$.
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fulltimeawaycut.pdf}
\caption{Plot of time $T(k^*_{hs},k_0;\ell_0)$ the wave packet takes to reach the hot spot region  at $k^*_{hs}$ starting away from the Hot spot at $k_0 = 6\Lambda$. $e = B_0 = 1$ and $\Lambda = 1$. The red curve correspond to the solution for the case $k_c>k_0$ and is given by Eqs. \eqref{eq:tepsilon} and Eq. \eqref{eq:thsk0}. The blue curve is given in the case $k_0>k_c$ by Eqs. \eqref{eq:tepsiloncold} and \eqref{eq:thskc}. For the latter curve, we can only trust until the Gray vertical line line at $\ell_0^* \approx 2.810$ where $\alpha_1(0) \approx 1$. The divergence before $\ell^*$ is due to the value $\ell_0 =1$, where the definitions of $v_0(0)$ and $\alpha_1(0)$ break down.}
\label{fig:fulltimezeroaway}
\end{figure}
Equivalently, we can write the last expression in terms of the bare scale $\ell_0$ and the scale $\ell^*_0$ given by
\begin{equation}
\left.\ell^*_0\right.^{\ell^*_0} = \exp\left(\frac{2\pi^2 N_c N_f}{N_c^2 - 1}\frac{k_0}{\Lambda}\right), 
\end{equation}
where $k_c=k_0$. Therefore,

Here the first term indicates that above $\ell^*_0 \approx 24.6403$ ($N_c = 2, N_f = 1, k_0 = 6\Lambda$) the Fermi velocity never reaches its saturation value across the whole integration region. The second term, when $\ell_0<\ell_0^*$, indicates that the integration region is divided in two parts separated by $k_c$: near the hot spot, where momentum is smaller than $k_c$, and the Fermi Velocity has a momentum profile; and away from the hot spot, with momentum larger than $k_c$ (but smaller than $k_0$), where the Fermi velocity reaches a saturation value of 1.


\subsubsection{$\alpha_1 \ll 1 $ and $\alpha_1 \approx 1$ limits near the Hot Spot}

In the case $0 < \varepsilon < k(t) < k^*_{hs} \ll k_c$, we have to consider the full flow:
\begin{equation}
\dot{k}(t) = -\frac{e B_0}{\mathcal{E}_1(\ell^{(2L)}_{k(t)};0)}, 
\quad \dot{k}_y(t) = \frac{e B_0 v_0(\ell^{(2L)}_{k(t)})}{\mathcal{E}_1(\ell^{(2L)}_{k(t)};0)}.
\label{eq:dotkeqfull}
\end{equation}
The new FS condition is
\begin{equation}
k_y(t) = -v_0(\ell^{(2L)}_{k(t)})k(t).
\end{equation}
The time $T_3$ it takes the wave packet to go from $k^*_{hs}$ to $\varepsilon$ is given by the integral
\begin{equation}
T_3(\varepsilon,k^*_{hs};\ell_0) = - \frac{1}{e B_0} \int_{k^*_{hs}}^{\varepsilon} \mathcal{E}_1(\ell^{(2L)}_k;0)\mathrm{d}k.
\label{eq:T3integral}
\end{equation}
We only consider this equation here since $k^*_{hs}$ is well below the cold momentum $k_c$, this is no necessary to consider a regime where $\mathcal{V}_F = 1$.

In the small momentum limit (since we are approaching the hot spot), we expand $\mathcal{E}_1(X;0)$ for large $X$:
\begin{equation}
\mathcal{E}_1(\ell^{(2L)}_k;0) \approx \nu(\ell_0)\exp\left(\sqrt{N_c^2-1}\frac{\sqrt{\ell^{(2L)}_{k}+\ell_0}}{\log\sqrt{\ell^{(2L)}_{k}+\ell_0}}\right),
\end{equation}
where
\begin{equation}
\nu(\ell_0) = \exp\left(-\sqrt{N_c^2-1}\Ei\left(\log\sqrt{\ell_0}\right)\right)
\end{equation}
is a constant in the $k$-integration. Changing variables in Eq. \eqref{eq:T3integral} to $s = \sqrt{\ell^{(2L)}_k+\ell_0}$ leads to
\begin{equation}
T_3(\varepsilon,k^*_{hs};\ell_0) =\frac{\Lambda e^{\ell_0}}{2 v_0(0)} \frac{\nu(\ell_0)}{e B_0} \int_{\sqrt{2\ell_0}}^{\sqrt{\log\left(\frac{\Lambda}{4 v_0(0)\varepsilon}\right)+\ell_0}}\exp\left(-s^2 + \sqrt{N_c^2-1}\frac{s}{\log s}\right) s \mathrm{d}s.
\label{eq:T3integrals}
\end{equation}
We are interested in the $\varepsilon\to 0$ limit, thus the integrals is
\begin{equation}
T_3(\varepsilon\to 0,k^*_{hs};\ell_0) =\frac{\Lambda e^{\ell_0}}{2 v_0(0)} \frac{\nu(\ell_0)}{e B_0} \int_{\sqrt{2\ell_0}}^{\infty}\exp\left(-s^2 + \sqrt{N_c^2-1}\frac{s}{\log s}\right) s \mathrm{d}s,
\label{eq:T3integralsinfty}
\end{equation}
for $\ell_0 > \ell^{\text{crit}}_0$\footnote{{\color{red} DOUBLE CHECK}Technically, we only have confidence of this result above the scale $\ell^{v;\text{crit}}_0$ where $v_0(0) \leq 1$. For $N_c=2, N_f=1$, $\ell^{v;\text{crit}}_0 \approx 2.9917 > \ell^{\text{crit}}_0$}. Obtaining a closed expression for the solution of the integral is hard, but we can obtain bounds fot $T_3(0,k^*_{hs};\ell_0)$,

The lower bound
\begin{equation}
T_3^{(l)}(0,k^*_{hs};\ell_0) = \frac{\nu(\ell_0)}{e B_0}k^*_{hs}
\label{eq:T3lowerbound}
\end{equation}
is given by dropping the $s/\log s$ term in the exponential of the integrals, while the upper bound
\begin{equation}
T_3^{(u)}(0,k^*_{hs};\ell_0) = \frac{\nu(\ell_0)}{e B_0}\left[e^{\frac{\sqrt{2(N_c^2-1)\ell_0}}{\log\sqrt{2\ell_0}}}k^*_{hs}+\frac{\sqrt{\pi(N_c^2-1)}}{4\log\sqrt{2\ell_0}}e^{\frac{N_c^2-1}{4\log^2\sqrt{2\ell_0}}}\frac{\Lambda e^{\ell_0}}{2 v_0(0)}\left(1+\text{erf}\left(\frac{\sqrt{N_c^2-1}}{2\log\sqrt{2\ell_0}}-\sqrt{2\ell_0}\right)\right)\right].
\label{eq:T3upperbound}
\end{equation}
is obtained by setting $\log s=\log\sqrt{2\ell_0}$. Numerically solving the integral in Eq. \eqref{eq:T3integralsinfty} we obtain a small finite time that increases with decreasing $\ell_0$ in the low energy regime ($\ell_0>\ell^{\text{crit}}_0$). This numerical plot, compared with the upper (green) and lower (orange) bounds can be seen in Fig. \ref{fig:T3HS}.


The total time a semi classical wave packet takes to reach the hot spot starting from $k_0$ is
\begin{equation}
T(0,k_0;\ell_0) = T_{12}(k^*_{hs},k_0;\ell_0) + T_3(0,k^*_{hs};\ell_0).
\end{equation}

%{\color{red} The formal solution of $k(t)$ is
%\begin{equation}
%\frac{k^*_{0} - k(t)}{e B_0} = \int_{t_0}^{t}\frac{\mathrm{d}t'}{\mathcal{E}_1(\ell^{(2L)}_{k(t')};0)},
%\end{equation}
%where $k(t_0) = k^*_{0} \leq k^*_{hs}$ is fixed and the final time is defined as $k(t_f) = \varepsilon$. 
%
%Let us start with the low energy limit, $\alpha_1(0) \ll 1$. Numerically, the solution of this equation indicates that the wave packet reaches the hot spot earlier as we take the low energy limit (See Fig. \ref{fig:timezeronear}).
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.75\linewidth]{zeroesLWkHS.pdf}
%\caption{Numerical plot of time $t^{(0)}_{hs}$ the wave packet takes to reach the hot spot in the region near the Hot spot. The fixed initial momentum is $k^*_{0} = 10^{-6} \Lambda$ and ``hot spot'' momentum is $k^*_{hs} \sim 1.8\times10^{-6}, \ldots, 1.4\times10^{-6}$ for the different values of $\ell_0$ and $k^*_{0}$. In contrast to the $k^*_{hs} < k$ case, here the wave packet takes less time to reach the hot spot as we move towards the small $v_0(0)$ limit.}
%\label{fig:timezeronear}
%\end{figure}
%Near the critical value $\alpha_1(0) \approx 1$, the wave packet takes more time to reach the hot spot as we approach this limit from below (Fig. \ref{fig:timezeroalpha1}) and less time if we approach from above (Fig. \ref{fig:timezeroalpha2}). The full plot can be seen in Fig. \ref{fig:timealpha12full}.}
%\begin{figure}[t]
%\centering
%\begin{subfigure}{0.49\linewidth}
%\includegraphics[width=\linewidth]{zeroesLWkHSalpha1.pdf}
%\caption{}
%\label{fig:timezeroalpha1}
%\end{subfigure}
%\begin{subfigure}{0.49\linewidth}
%\includegraphics[width=\linewidth]{zeroesLWkHSalpha2.pdf}
%\caption{}
%\label{fig:timezeroalpha2}
%\end{subfigure}
%\caption{Time the wave packet takes to reach the hot spot in the region near the Hot spot (a) approaching the critical value $\alpha_1(0) \approx 1$ from below and (b) approaching $\alpha_1(0) \approx 1$ from above.}
%\label{fig:timealpha12}
%\end{figure}
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.6\linewidth]{zeroesLWkHSalpha12.pdf}
%\caption{Time the wave packet takes to reach the hot spot in the region near the Hot spot for different values of $\ell_0$. The origin is located at ($\ell_0 = 2.810$,$0.0$)}
%\label{fig:timealpha12full}
%\end{figure}

==> referee <==
----------------------------------------------------------------------
Report of the First Referee -- XF10756B/Borges
----------------------------------------------------------------------

The authors of the manuscript "Emergence of curved momentum-spacetime 
and its effect on the cyclotron motion in the antiferromagnetic 
quantum critical metal" show that the low-energy theory of a metal 
with antiferromagnetic spin fluctuations can be captured by a curved 
momentum-spacetime. The critical spin fluctuations around nesting 
hotspots on the Fermi surface give rise to the slowdown of the 
quasiparticles close to these hotspots. The authors calculate the 
cyclotron period in this scenario and identify the analogies between 
this condensed matter context and the theory of general relativity. In 
particular, they propose the condensed matter realization of some 
effects near a black hole horizon like the frozen motion of the 
quasiparticles in a semiclassical picture of the cyclotron motion. 

Whereas the overall result is fascinating and can be considered as 
worth to be published, the presented manuscript has various weaknesses 
that let me conclude that major corrections are required before that I 
can recommend it for publication. I will justify my conclusion in the 
following with concrete remarks and questions that may help to improve 
the quality of the manuscript. 

1. There is a very strong imbalance between the manuscript length for 
the new physical results and the presentation of the concepts 
necessary to understand these new results. The presentation of the 
necessary concepts is nevertheless incomplete. To be precise: 

1a. The review of the theory of the antiferromagnetic quantum critical 
metal in Section II is very complicated and very lengthy. In my 
understanding, the key new result of the paper starts at page 8 around 
equation (16). The authors should generally streamline their review to 
the essentials only. Further details might be provided in some 
appendix. Just to mention a few examples: The statement of the model 
in Eq (1), the generality of the approach (arbitrary spin and 
flavor), and the details of the RG around Eq (5) or (9) are extremely 
complicated and hide the key messages. It remains unclear how these 
aspects in this depth are relevant for the new results of the 
manuscript. Furthermore, it remains unclear if there are new insights 
in this part or if it is essentially published in Ref. [14]. 

1b. It might be very helpful to present the results for a selection of 
segments only and explain the remaining segments in an appendix. It is 
particular important to focus on one choice only. In the presented 
manuscript the authors permanently change the segments that they 
consider. 

1c. Some notations are confusing and misleading. For instance, mu is 
usually used as chemical potential and its value (or the particle 
filling) is essential in the analysis of the mentioned physical 
systems. The letter v used for the nesting angle is usually used as 
quasiparticle velocity. The authors should adjust their notation so 
that confusions are reduced to a minimum. 

1d. Whereas some aspects are presented too detailed, other concepts 
are barely reviewed. In particular, the presentation around Eq (4) 
uses objects that are never precisely defined, the derivation of Eq 
(6) is not presented and the relevant scales are defined and explained 
at various different places or in the footnote only. A review on the 
used concepts of curved space time are missing and should be added. I 
suggest to present the bare minimum only and refer to the 
corresponding references for more details. If some steps are indeed 
needed for the original results, they should be presented in 
sufficient detail to be reproducible. 

2. The results and its physical interpretation remain intransparent in 
several respects. This is a major downside since it remains partially 
unclear in which sense the presented theory is valid, useful, and can 
be applied elsewhere. Furthermore, the gain of new insights in the 
presented example is not obvious. Several statements need further 
precise calculations to show their validity. To be precise: 

2a. Most importantly, the authors need to include more explicit 
calculations for their new results starting on page 8. Many 
derivations of the key results are not presented or not presented in 
sufficient detail. For instance, the steps to derive Eq (16) from Eq. 
(14) should be presented very detailed. How does the mapping precisely 
work? Other examples are: How are the scaling behavior of the vielbein 
calculated in the various cases? The derivation for the 
temperature-dependent case as well as the superconducting case are 
essentially missing. I do not find any detailed discussion about the 
torsion and its relevance here, how Eq (17) and (19) are derived, how 
the authors came to their conclusions below Eq (20), how the mapping 
to the Schwarzschild black hole is performed and how footnote 11 is 
justified. The reduction of details in the first part of the 
manuscript will provide space for more detailed derivations and 
discussions of their original results. 

2b. The authors focus on one type of quantum criticality, namely 
antiferromagnetic quantum criticality. Does their theory also apply to 
other types of quantum criticality? 

2c. How are the presented results related to the existing models of 
cuprates or the other systems that the authors intend to describe? Can 
the authors make predictions for specific compounds? 

2d. It would be useful to summarize the key assumptions, notations, 
mappings, fixed scales more prominently. Examples are: A summary of 
the two ways to fix the unit of frequency (the clock) and its 
interpretation. The existing figures 1 to 5 give some impressions but 
are partially confusing and do not contain all essential information. 
Examples are the compactification of the imaginary time in Fig 5, 
footnote 4 in combination with Fig 3, the definition of the different 
length scales in Fig 3 that could also be included into the other 
figures, the diagrams and the introduction of delta E in Fig 2 that 
are never used explicitly throughout the manuscript. Other important 
aspects and their interpretation do not have any representation in 
figures like the torsion or the relation to general relativity. It 
would be nice to make the definition and concept of nesting angle more 
prominent due to its importance throughout the manuscript. 

2e. The relevance of the other figures is questionable. It is hardly 
possible to gain any insights just by considering Fig 6, 8, 9 and 10. 
The authors should highlight precisely in the caption and in the main 
text why they are presenting precisely these aspects for their choices 
of parameters. It remains unclear how the curves are precisely 
calculated. 

2f. The assumption in footnote 9 is highly confusing. The authors 
should explicitly show that the final result is not affected by this 
assumption. 

2g. The manuscript needs much more connection to existing literature 
of quantum criticality and transport therein. The authors should 
precisely compare their perspective to the existing literature. Are 
the results consistent? What are the new aspects that we can 
understand better by changing the perspective? How does the spacetime 
mapping look like in basic limits? I would expect that the 
semiclassical description breakdowns down around the quantum critical 
point. Thus, how reliable are the results of semiclassical transport 
theory? What is the impact of loosing quasiparticle weight and low 
quasiparticle lifetime near the hotspots? 

3. I have several additional questions and comments: 

3a. The authors mention that the momentum-dependent red shift is the 
primary mechanism by which the Fermi velocity acquires a strong 
momentum dependence in the presented context. What are other effects 
and in which sense could it or could it not be captured by the curved 
momentum-spacetime geometry picture? 

3b. It might be interesting to present an outlook how the presented 
geometric perspective could be related to other recent developments, 
for instance, in the context of emergent gravity in semiclassical 
transport (arXiv:2111.07782) or for cyclotron motion in systems with 
unconventional bands crossings like in non-Hermitian systems 
(PhysRevB.104.L201107), moire superlattices (PhysRevLett.130.066001) 
or chiral magnets (Nature volume 594, pages 374–379 (2021)). 

3c. I suggest to reduce the number of footnotes. 

3d. The authors should elaborate on the significance of the references 
for their work in the large list of references from 19 to 40. 

3e. To the best of my knowledge, none of the references in 41 to 51 is 
actually using the concept of curved momentum-spacetime geometry. They 
are studies of the cyclotron motion of quasiparticles. As presented, 
the combination of the sentence and the list of references is 
misleading and should be clarified.

----------------------------------------------------------------------
Report of the Second Referee -- XF10756B/Borges
----------------------------------------------------------------------

The authors compute the renormalized electron dispersion in a 
two-dimensional antiferromagnetic quantum critical metal and 
reformulate its strong momentum dependence as an emergent curved 
momentum-spacetime. They then compute the cyclotron period from a 
semiclassical electron dynamics in the curved momentum-spacetime 
picture. An interesting non-monotonic dependence on the bare nesting 
angle is obtained. 

The renormalized dispersion has already been derived earlier by the 
second author and coworkers. The curved momentum-spacetime 
interpretation and the calculation of the cyclotron period seem new to 
me, and are both interesting. 

However, it is not clear to me whether the change of variables leading 
to the curved spacetime picture makes calculations easier. More 
specifically, would the calculation of the cyclotron period be harder 
in the standard reference frame? If not, the authors should say which 
other advantages are obtained from their unconventional point of view. 

Besides the above remark, I have only some remarks on the 
presentation. 

1) Sec. II contains a fairly long review of the calculation of the 
renormalized dispersion, and a shorter part on the geometric 
description in a curved spacetime. For a better orientation of the 
reader, one might divide this section in two subsections. 

2) I was confused by the notation v_k for the nesting angle, since v_k 
is usually used to denote the velocity of particles. And using a 
capital V_F for the Fermi velocity is also unusual, usually it's v_F . 
If their notation is in line with previous work on the topic, the 
authors may like to keep it as it is. Otherwise they could adopt a 
better notation. 

3) I think that \bar N in Eq. (1) has not been defined. 

4) In the caption to Fig. 3 there is a “and one-loop fermion” too 
much. 

In summary, I recommend publication in PRB after the authors have 
addressed the above comments.

